Derandomizing Multi-Distribution Learning

Multi-distribution or collaborative learning involves learning a single predictor that works well across multiple data distributions, using samples from each during training. Recent research on multi-distribution learning, focusing on binary loss and finite VC dimension classes, has shown near-optimal sample complexity that is achieved with oracle efficient algorithms. That is, these algorithms are computationally efficient given an efficient ERM for the class. Unlike in classical PAC learning, where the optimal sample complexity is achieved with deterministic predictors, current multi-distribution learning algorithms output randomized predictors. This raises the question: can these algorithms be derandomized to produce a deterministic predictor for multiple distributions? Through a reduction to discrepancy minimization, we show that derandomizing multi-distribution learning is computationally hard, even when ERM is computationally efficient. On the positive side, we identify a structural condition enabling an efficient black-box reduction, converting existing randomized multi-distribution predictors into deterministic ones.

==> fixed_algo_arxiv.tex <==
\section{Deterministic multi-distribution learner}
In this section, we give our algorithm for derandomizing multi-distribution learners for label-consistent distributions, i.e.\ we assume $\cD_i(y \mid x) = \cD_j(y \mid x)$ for all $i,j,x$.

We start by presenting the high level ideas of our algorithm. First, consider running any of the previous randomized multi-distribution learners, producing a distribution $F$ over hypotheses in $\cH$ satisfying $\max_i \E_{f \sim F}[\er_{\cD_i}(f)] \leq \tau + \eps/2$. Consider randomly rounding this distribution to a deterministic classifier $\hat{f}$ as follows: For every $x \in \cX$ independently, sample an $f \sim F$ and let $\hat{f}(x)=f(x)$. For any distribution $\cD_i$, we clearly have $\E[\er_{\cD_i}(\hat{f})]=\E[\er_{f \sim F}(h)] \leq \tau + \eps/2$. However, as also discussed in the introduction, it is not clear that we can union bound over all $k$ distributions and argue that $\er_{\cD_i}(\hat{f}) \leq \tau + \eps$ for all of them simultaneously. Notice however that the independent choice of $\hat{f}(x)$ for each $x$ gets us most of the way. Indeed, if we let $Z_x$ be a random variable (determined by $\hat{f}(x)$) giving $\Pr_{y \sim \cD(y \mid x)}[\hat{f}(x) \neq y]$, then $\er_{\cD_i}(\hat{f}) = \sum_{x \in \cX} \cD_i(x)Z_x$, where $\cD_i(x)$ denotes the probability of $x$ under $\cD_i$ and $\cD_i(y \mid x)$ gives the conditional distribution of the label $y$ given $x$. Now notice that $\cD_i(x)Z_x$ is a random variable taking values in $[(1/2-\beta_x)\cD_i(x), (1/2+\beta_x)\cD_i(x)]$ where $\beta_x = 1/2 + \cD_1(1 \mid x)$ denotes the \emph{bias} of the label of $x$. Here $\cD_1(1 \mid x)$ is just the probability of seeing the label $1$ on $x$. Furthermore, these random variables are independent. We also have $\E[\er_{\cD_i}(\hat{f})] =\E_{f \sim F}[\er_{\cD_i}(f)]$. Thus by Hoeffding's inequality
\[
\Pr[|\er_{\cD_i}(f) - \E_{f \sim F}[\er_{\cD_i}(f)]| > \eps/2] < 2\exp\left(-\frac{\eps^2}{2 \cdot \sum_{x \in X} (2 \beta_x \cD_i(x))^2}\right).
\]
Examining this expression closely, we observe that this probability is small if $\beta_x \cD_i(x)$ is small for all $x \in \cX$. 

Using this observation, our algorithm then starts by drawing $\tilde{O}(\eps^{-2})$ samples from each distribution $\cD_i$ and collecting all observed $x \in X$ in a set $T$. Importantly, with good probability, $T$ contains all $x \in X$ with $\beta_x^2 \cD_i(x)=\tilde{\Omega}(\eps^2)$ for at least one $i$. The idea now is that every element $x \notin T$ has a small $\beta_x^2 \cD_i(x)$ for all $i$, and hence we can afford to choose $\hat{f}(x)$ randomly for these $x$ by Hoeffding.

What remains is then to handle the points in $T$. Here we basically exploit that we have enough samples to correctly determine $\sign(\beta_x)$ for all these $x$. Hence we make perfect predictions on $x \in T$. Here we are crucially exploiting that $\cD_i(y \mid x) = \cD_j(y \mid x)$ for all $i,j,x$.

In summary, our algorithm first gathers all $x \in X$ that have a large probability $\beta_x \cD_i(x)$ under some $\cD_i$. We then estimate the most likely label for each such $x$ and let $\hat{f}(x)$ predict this label. For all $x \notin T$, we randomly decide on $\hat{f}(x)$ by independently drawing an $f \sim F$ and letting $\hat{f}(x)=f(x)$. The algorithm is shown as Algorithm~\ref{alg:simple}.

\input{alg_determ_fixed}

Before giving the formal analysis of the algorithm, note that storing the classifier $\hat{f}$ is quite expensive, as we need to remember the random choice of $\hat{f}(x)$ for every $x \in \cX \setminus T$. This is one place where we use the assumption that $\cX$ is finite. Note however that even for finite $\cX$, storing $|\cX|$ random choices to represent the classifier might be infeasible. We propose a method for reducing the storage requirement later in this section. For now, we analyse Algorithm~\ref{alg:simple} without worrying about storage of $\hat{f}$.

\paragraph{Analysis.}
In our analysis, we separately handle $x \in T$ and $x \notin T$. The two technical results we need are stated next. First, define the \emph{bias} $\beta_x$ of an $x \in \cX$ as $\cD_1(1 \mid x) - 1/2$. That is, $\beta_x = \E_{y \sim \cD_1(y \mid x)}[y]$. We say that an $x$ is \emph{heavily biased} if 
\[
\beta_x^2 \cD_i(x) > \frac{\eps^2}{8 \cdot \ln(4k/\delta)}
\]
for at least one $i$, and \emph{lightly biased} otherwise. Intuitively, our algorithm ensures that $T$ contains all heavily biased $x$ and that all predictions made on $x \in T$ are correct. This is stated in the following
\begin{lemma}
\label{lem:heavy}
It holds with probability at least $1-\delta/4$ that every heavily biased $x$ is in $T$, and furthermore, for every $x \in T$, we have $\hat{f}(x) = \sign(\beta_x)$.
\end{lemma}

\begin{lemma}
\label{lem:light}
Assume every heavily biased $x$ is in $T$ after step 8. Then with probability at least $1-\delta/4$ over the random choice of $\hat{f}(x)$ with $x \in \cX \setminus T$, it holds for all $i$ that
\[
\left|\E_{f \sim F}[\E_{(x,y) \sim \cD_i}[1\{x \notin T \wedge f(x) \neq y\}]] - \E_{(x,y) \sim \cD_i}[1\{x \notin T \wedge \hat{f}(x) \neq y\}]\right| \leq \eps/2.
\]
\end{lemma}


Before giving the proof of \cref{lem:heavy} and \cref{lem:light}, let us use these two results to complete the proof of \cref{thm:algo}. 
\begin{proof}[Proof of \cref{thm:algo}]
From a union bound and \cref{lem:heavy} and \cref{lem:light}, we have with probability $1-\delta$ that all of the following hold
\begin{itemize}
    \item The invocation of $\cA$ in step 1 of Algorithm~\ref{alg:simple} returns a distribution $F$ with $\max_i \E_{f \sim F}[\er_{\cD_i}(f)] \leq \tau + \eps/2$.
    \item For every $x \in T$, we have $\hat{f}(x) = \sign(\beta_x)$.
    \item For every distribution $\cD_i$, \[
\left|\E_{f \sim F}[\E_{(x,y) \sim \cD_i}[1\{x \notin T \wedge f(x) \neq y\}]] - \E_{(x,y) \sim \cD_i}[1\{x \notin T \wedge \hat{f}(x) \neq y\}]\right| \leq \eps/2.
\]
\end{itemize}
Assume now that all of the above holds. We rewrite $\er_\cP(\hat{f})$ by splitting the contributions to the error into $x \in T$ and $x \notin T$
\begin{eqnarray*}
    \er_\cP(\hat{f}) &=& \max_i \er_{\cD_i}(\hat{f})\\
    &=& \max_i \left(\E_{(x,y)\sim \cD_i}[1\{x \in T \wedge \hat{f}(x)\neq y\}] + \E_{(x,y) \sim \cD_i}[1\{x \notin T \wedge \hat{f}(x) \neq y\}]\right).
\end{eqnarray*}
Using that $\hat{f}(x) = \sign(\beta_x)$ for $x \in T$, we have $\E_{(x,y)\sim \cD_i}[1\{x \in T \wedge \hat{f}(x)\neq y\}] = \min_{z \in \{-1,1\}^T}[\E_{\cD_i}[1\{x \in T \wedge z(x)\neq y\}]$. Thus the above is bounded by
\begin{eqnarray*}
    \max_i \left(\min_{z \in \{-1,1\}^T}[\E_{\cD_i}[1\{x \in T \wedge z(x)\neq y\}] + \E_{f \sim F}[\E_{\cD_i}[1\{x \notin T \wedge f(x) \neq y\}]]\right) + \eps/2.
\end{eqnarray*}
Since every $f$ in the support of $F$ is a deterministic classifier, we have 
\begin{eqnarray*}
    \min_{z \in \{-1,1\}^T}[\E_{\cD_i}[1\{x \in T \wedge z(x)\neq y\}] \leq
    \E_{f \sim F}[\E_{\cD_i}[1\{x \in T \wedge f(x)\neq y\}].
\end{eqnarray*}
We therefore have
\begin{eqnarray*}
    \er_\cP(\hat{f}) &\leq&  \\
    \max_i \left(\E_{f \sim F}[\E_{\cD_i}[1\{x \in T \wedge f(x)\neq y\}]]+ \E_{f \sim F}[\E_{\cD_i}[1\{x \notin T \wedge f(x) \neq y\}]]\right) + \eps/2&=&\\
    \max_i \E_{f \sim F}[\er_{\cD_i}(f)] + \eps/2 &\leq& \\
    \tau + \eps.
\end{eqnarray*}
This completes the proof of \cref{thm:algo}.
\end{proof}

\begin{proof}[Proof of \cref{lem:heavy}]
For short, let $\alpha = \eps^2/(\sqrt{C}\ln \gamma)$ and note that $\alpha m = \sqrt{C} \ln \gamma$ is the threshold used in step 6 of Algorithm~\ref{alg:simple}. We define a number of failure events.
\begin{itemize}
\item For every $i$ and every $x$ with $\cD_i(x) \geq 2\alpha$, let $E^1_{i,x}$ be the event that $x$ is not added to $T_i$ in step 6 of iteration $i$ of the for-loop. 
\item For every $i$ and every $x$ with $\cD_i(x) < \alpha/e^2$, let $E^2_{i,x}$ be the event that $x$ is added to $T_i$ in step 6 of iteration $i$ of the for-loop.
\item For every $i$ and every $x$ with $\cD_i(x) \geq \alpha/e^2$, let $E^3_{i,x}$ denote the event that $|V_{i,x}| \notin [\cD_i(x)m/2, 2\cD_i(x)m]$.
\item For every $i$ and every $x$ with $\cD_i(x) \geq \alpha/e^2$, let $E^4_{i,x}$ denote the event that $|\rho_{i,x} - (1/2 + \beta_x)| > \sqrt{\ln(\gamma)/|V_{i,x}|}$.

\end{itemize}
Assume first that none of the events $E^j_{i,x}$ occur. Consider a heavily biased $x$. Then there is an $i$ for which $\cD_i(x) > \eps^2/(8 \ln(4k/\delta)) > 2\alpha$, where the last inequality holds for $C$ large enough. Since $E^1_{i,x}$ does not occur, $x$ is added to $T_i$ in step 6 of iteration $i$ of the for-loop. Since $E^4_{i,x}$ does not occur we have $|\rho_{i,x} - (1/2 + \beta_x)| \leq \sqrt{\ln(\gamma)/|V_{i,x}|}$. Since $E^3_{i,x}$ does not occur and $x$ is heavily biased, we also have $\beta_x > \sqrt{\eps^2/(8 \cD_i(x) \ln(4k/\delta))} > \sqrt{(C/8)\ln(\gamma)/(\cD_i(x)m)} > \sqrt{(C/16)\ln(\gamma)/|V_{i,x}|}$. For $C$ large enough, we thus have $|\rho_{i,x} - 1/2| \geq |\beta_x|-\sqrt{\ln(\gamma)/|V_{i,x}|} > \sqrt{\ln(\gamma)/|V_{i,x}|}$. Hence $x$ remains in $T_i$ during step 7 of iteration $i$ of the for-loop. We have thus shown that every heavily biased $x$ is in $T$. Next, consider an arbitrary $x$ that remains in $T_i$ during step 7 of iteration $i$ of the for-loop. Then $\rho_{i,x} \notin [1/2-\sqrt{\ln(\gamma)/|V_{i,x}|}, 1/2 + \sqrt{\ln(\gamma)/|V_{i,x}|}]$. Also, since $E^2_{i,x}$ did not occur, we know $\cD_i(x) \geq \alpha/e^2$. Thus by the arguments above, we also have $|\rho_{i,x} - (1/2 + \beta_x)| \leq \sqrt{\ln(\gamma)/|V_{i,x}|}$. This implies that $\rho_{i,x} - 1/2$ and $\beta_x$ have the same sign and thus $\hat{f}(x) = \sign(\beta_x)$.

All that remains is thus to show that $\Pr[\cup E^j_{i,x}] \leq \delta/4$.

For $E^1_{i,x}$, consider an $x$ with $\cD_i(x) \geq 2 \alpha$. The expected number of samples $(x',y')$ with $x'=x$ in $S_i$ is $\cD_i(x) m \geq 2 \alpha m = 2\eps^2 m/(\sqrt{C}\ln \gamma) = \sqrt{C} \ln \gamma$. It follows from a Chernoff bound that $\Pr[E^1_{i,x}] \leq \gamma^{-2}$ for $C$ large enough. 

For $E^2_{i,x}$, consider an $x$ with $\cD_i(x) < \alpha/e^2$. By a Chernoff bound, we have that the probability that $x \in T_i$ after step 5 is no more than 
\[
\left(\frac{e^{\alpha/\cD_i(x)-1}}{(\alpha/\cD_i(x))^{\alpha/\cD_i(x)}} \right)^{\cD_i(x) m} \leq \left(e\cD_i(x)/\alpha\right)^{\alpha m}.
\]
A union bound over all such $x \in \cX$ gives 
\begin{eqnarray*}
\Pr[\cup_{x} E^2_{i,x}] &\leq& \sum_{x \in \cX : \cD_i(x) < \alpha/e^2} (e\cD_i(x)/\alpha)^{\alpha m} \\
&\leq& \sum_{x \in \cX : \cD_i(x) < \alpha/e^2} e^{-\alpha m+1} (e\cD_i(x)/\alpha) \\&\leq& e^{-\alpha m+2}/\alpha.
\end{eqnarray*}
By our choice of $\alpha = \eps^2/(\sqrt{C} \ln \gamma)$ and $\alpha m = \sqrt{C} \ln \gamma$, we thus have for every $i$ that $\Pr[\cup_{x} E^2_{i,x}] \leq \gamma^{-2}$ for $C$ large enough.

For $E^3_{i,x}$, consider an $x$ with $\cD_i(x) \geq \alpha/e^2$. By Chernoff, we have $\Pr[E^3_{i,x}] \leq \exp(-\alpha m/(12 e^2)) = \exp(-\sqrt{C} \ln(\gamma)/(12 e^2))$. This is less than $\gamma^{-2}$ for $C$ large enough.

For $E^4_{i,x}$, consider an $x$ with $\cD_i(x) \geq \alpha/e^2$. Conditioned on $|V_{i,x}|$, we have that $\E[\rho_{i,x}] = 1/2 + \beta_x$. By Hoeffding's inequality, we get $\Pr[|\rho_{i,x} - (1/2 + \beta_x)| > \sqrt{\ln(\gamma)/|V_{i,x}|}] < 2\exp(-2\ln(\gamma)) \leq 2\gamma^{-2}$. Since this holds for all $|V_{i,x}|$, we conclude $\Pr[E^4_{i,x}] \leq 2 \gamma^{-2}$.

The number of events $E^1_{i,x}, E^3_{i,x}, E^4_{i,x}$ is no more than $3 k e^2 \alpha^{-1} = 3 e^2 \sqrt{C} k \eps^{-2} \ln \gamma$. Since each of them occur with probability at most $2 \gamma^{-2}$, we have 
\[
\Pr[\cup E^j_{i,x}] \leq \gamma^{-2} 6 e^2 \sqrt{C} k \eps^{-2} \ln \gamma + \gamma^{-2} \leq \delta/4,
\]
for $C$ large enough.
\end{proof}


\begin{proof}[Proof of \cref{lem:light}]
Fix a distribution $\cD_i$. Observe that for any $x \in \cX \setminus T$, we have that the distribution of $\hat{f}(x)$ is the same as $f(x)$ for $f \sim F$. Hence $\E_{\hat{f}}[\E_{(x,y) \sim \cD_i}[1\{x \notin T \wedge \hat{f}(x) \neq y\}]] = \E_{f \sim F}[\E_{(x,y) \sim \cD_i}[1\{x \notin T \wedge f(x) \neq y\}]]$. Denote this expectation by $\mu$. If we let $Z_x$ be the random variable (as a function of $\hat{f}(x)$) taking the value $\Pr_{\cD_i(y \mid x)}[\hat{f}(x) \neq y]$, then
\[
\E_{(x,y) \sim \cD_i}[1\{x \notin T \wedge \hat{f}(x) \neq y\}] = \sum_{x \in \cX \setminus T} \cD_i(x)Z_x.
\]
Observe that $Z_x$ is either $1/2-|\beta_x|$ or $1/2+|\beta_x|$, depending on whether $\hat{f}(x) = \sign(\beta_x)$ or not. Hence $\cD_i(x)Z_x \in [\cD_i(x)(1/2-|\beta_x|), \cD_i(x)(1/2+|\beta_x|)]$ and the $Z_x$ are independent. We thus get from Hoeffding's inequality and that $x \notin T$ are lightly biased that
\begin{eqnarray*}
\Pr_{\hat{f}}\left[\sum_{x \in \cX \setminus T} \cD_i(x)Z_x > \mu+\eps/4\right] &<& \exp\left(\frac{-2(\eps/2)^2}{\sum_{x \in \cX \setminus T} (2|\beta_x|\cD_i(x))^2} \right) \\
&\leq& \exp\left(\frac{-\eps^2}{\sum_{x \in \cX \setminus T} \cD_i(x) \eps^2/\ln(4k/\delta)} \right)\\
&\leq& \exp\left(-\ln(4k/\delta) \right)\\
&=& \delta/(4k).
\end{eqnarray*}
A union bound over all $\cD_i$ completes the proof.
\end{proof}





\subsection{Reducing Storage}
The above description of Algorithm~\ref{alg:simple} requires the storage of an independent random choice of $\hat{f}(x)$ for every $x \in \cX$. This is infeasible for large $\cX$. Instead, we can reduce the storage requirements by  using an $r$-wise independent hash function $q : \cX \to \cY$ for a sufficiently large output domain $\cY$ to make the random rounding. Concretely, such a hash function can be implemented in space $O(r \lg (|\cX||\cY|))$ bits and evaluated in time $\tilde{O}(r \lg(|\cX||\cY|))$ by e.g.\ interpreting an $x \in \cX$ as an index into $[|\cX|] = \{0,\dots,|\cX|-1\}$ and letting $q(x) = \sum_{i=0}^{r-1} \alpha_i x^i \bmod p$ for a prime $p > \max\{|\cX|,|\cY|\}$ and the $\alpha_i$ independent and uniform random in $[p]$. Using fast multiplication algorithms, $q(x)$ can be evaluated in time $\tilde{O}(r \lg(|\cX||\cY|))$.

The learning algorithm now stores $q$ as well as the distribution $F$. Given this information, we compute $\hat{f}(x)$ by computing $q(x)$ and letting $\hat{f}(x) = 1$ if $q(x) > (1/2 + \E_{f \sim F}[f(x)]/2)p$ and $0$ otherwise. If $p$ (and thus $|\cY|$) is large enough, this essentially rounds $\hat{f}(x)$ with the same probabilities as Algorithm~\ref{alg:simple}. Since previous multi-distribution learning algorithms also store $F$, this only adds $O(r \lg(|\cX||\cY|))$ bits to the storage.

What remains is to determine an $r$ for which this is sufficient for the guarantees of Algorithm~\ref{alg:simple}. We will show that $r = O(\ln(k/\delta)/\eps)$ suffices. Here we only give an outline of how to modify the proof in the previous section to work with $r$-wise independence. First, redefine the threshold $\cD_i(x) > \eps^2/(8 \ln(4k/\delta))$ used in the definition of $T$. If we increase the number of samples $m$ by a $C'\ln(k/\delta)$ factor for a big enough constant $C'$, then we can require every $x$ with $\cD_i(x) > \eps^2/(C'' \ln^2(k/\delta))$ for some $i$ to be in $T$. Here $C''$ is a constant that grows with $C'$. Let $\alpha = \eps^2/(C'' \ln^2(k/\delta))$. The proof of \cref{lem:heavy} still goes through with this modified definition. The only step in the analysis that depends on the random rounding, is the proof of \cref{lem:light}. Here we use the following variant of the Hoeffding bound for random variables with limited independence
\begin{theorem}[\cite{}]
\label{thm:con}
Let $Z_1,\dots,Z_n$ be a sequence of $r$-wise independent random variables for $r \geq 2$ with $|Z_i - \E[Z_i]| \leq 1$ for all outcomes. Let $Z = \sum_i Z_i$ with $\E[Z]=\mu$ and let $\sigma^2(Z) = \sum_i \sigma^2(Z_i)$ denote the variance of $Z$. Then the following holds for even $r$ and any $C \geq \max\{r,\sigma^2(Z)\}$:
\[
\Pr[|Z-\mu| \geq T] \leq \left(\frac{rC}{e^{2/3}T^2}\right)^{r/2}.
\]
\end{theorem}
If we repeat the proof of \cref{lem:light}, define $Z_x$ as the random variable taking the value $\Pr_{\cD_i(y \mid x)}[\hat{f}(x) \neq y]$. We have $\cD_i(x) \leq \alpha$ for all $x \notin T$. Then
\[
\E_{(x,y) \sim \cD_i}[1\{x \notin T \wedge \hat{f}(x)\neq y\}] = \sum_{x \in \cX \setminus T} \cD_i Z_x = \alpha \sum_{x \in \cX \setminus T} \frac{\cD_i(x)  Z_x}{\alpha}. 
\]
Every random variable in this sum takes values in $[0,1]$ by definition of $\alpha$. We also have $\sigma^2(\cD_i(x)Z_x/\alpha) \leq (\cD_i(x)/\alpha)^2$ and thus
\[
\sigma^2\left(\sum_{x \in \cX \setminus T} \frac{\cD_i(x)Z_x}{\alpha}\right) \leq \sum_{x \in \cX \setminus T} \left(\frac{\cD_i(x)}{\alpha} \right)^2 = \left(\frac{1}{\alpha}\right)^2 \sum_{x \in \cX \setminus T} \cD_i(x)^2 \leq \frac{1}{\alpha}.
\]
Now let $r = \sqrt{1/\alpha} = \Theta(\sqrt{C''}\ln(k/\delta)/\eps)$. By \cref{thm:con} with $C = \sqrt{1/\alpha} = 1/(\alpha r)$, we get for $\mu = \E_{f \sim F}[\E_{(x,y) \sim \cD_i}[1\{x \notin T \wedge f(x) \neq y\}]]$ that
\[
\Pr\left[\left| \sum_{x \in \cX \setminus T} \frac{\cD_i(x) Z_x}{\alpha} - \mu/\alpha \right|  \geq T\right] \leq \left(\frac{rC}{e^{2/3}T^2}\right)^{r/2},
\]
and thus 
\[
\Pr\left[\left| \sum_{x \in \cX \setminus T} \cD_i(x) Z_x - \mu \right|  \geq \alpha T\right] \leq \left(\frac{rC}{e^{2/3}T^2}\right)^{r/2}.
\]
Inserting $T=\eps/(5 \alpha)$ finally implies
\begin{eqnarray*}
\Pr\left[\left| \E_{(x,y) \sim \cD_i}[1\{x \notin T \wedge \hat{f}(x) \neq y\}] - \E_{f \sim F}[\E_{(x,y) \sim \cD_i}[1\{x \notin T \wedge f(x) \neq y\}]] \right|  \geq \eps/5\right] &\leq\\
\left(\frac{25 rC \alpha^2}{e^{2/3}\eps^2}\right)^{r/2} \leq
\left(\frac{25 \alpha}{e^{2/3}\eps^2}\right)^{r/2} =
\left(\frac{25}{e^{2/3}C'' \ln^2(k/\delta) \eps^2}\right)^{r/2} \leq
2^{-r/2} \leq
\delta/(4k).
\end{eqnarray*}
Thus if we increase the sample complexity to $m(k,d,\tau,\eps/5,\delta/2) + O(k\ln^3(k/(\eps \delta))/\eps^2)$, then we may store a hash function using $O(\lg^2(n/\delta) \lg(|\cX||\cY|)/\eps)$ bits.
